Bottomonium spectroscopy using Coulomb plus linear (Cornell) potential

The coulomb plus linear (Cornell) potential is used to investigate the mass spectrum of bottomonium. Gaussian wave function is used in position and momentum space to estimate values of potential and kinetic energies, respectively. Based on our calculations, we study newly observed ${{\mathit \Upsilon}{(10860)}}$ as an admixture of $4^{3}S_{1}$ with $4^{3}D_{1}$, and ${{\mathit \Upsilon}{(10753)}}$ as an admixture of $6^{3}S_{1}$ with $4^{3}D_{1}$ also, we try to assign ${{\boldsymbol \Upsilon}{(11020)}}$ as a pure $4^{3}D_{1}$ bottomonium state. We also study the Regge trajectories in the $(J,M^{2})$ and $(n_r,M^{2})$ planes to help prove our association. We estimate the pseudoscalar and vector decay constants, the radiative (Electric and Magnetic Dipole) transition rates, and the annihilation decay width for bottomonium states.

==> com_mas_spect.tex <==
\begin{table*}
	
	\begin{centering}
		\caption{Complete mass spectra(in GeV).\label{tab:massesbb}}
		\par\end{centering}
	\centering{}%
	\scalebox{0.95}{
		\begin{tabular}{llllllllllll}
			\hline
			\addlinespace[3pt]
			\multirow{2}{*}{State} & \multirow{2}{*}{$J^{P}$} & This & Expt. &  \multicolumn{6}{c}{Others}\tabularnewline
			\addlinespace[2pt]
			\cline{5-12}
			\addlinespace[2pt]
			&  & work & Ref.~\cite{PDG:2020} &Ref.~\cite{Wang:2018} & Ref.~\cite{Bhat:2017} & Ref.~\cite{Deng:2017} & Ref.~\cite{Lu:2016mbb} & Ref.~\cite{Segovia2016} & Ref.~\cite{Godfrey:2015} & Ref.~\cite{Wurtz:2015} & Ref.~\cite{Li:2009nr} \tabularnewline
			\addlinespace[2pt]
			\hline
			\addlinespace[3pt]
			$1^{1}S_{0}$ & $0^{-+}$ & 9.423 & 9.399 &9.398& 9.400  &  9.390 & 9.395 & 9.455 & 9.402  & 9.402 & 9.389 \tabularnewline
			$1^{3}S_{1}$ & $1^{--}$ & 9.463 & 9.460 &9.463& 9.461  & 9.460 & 9.459 & 9.502  & 9.465  & 9.460 & 9.460 \tabularnewline
			$2^{1}S_{0}$ & $0^{-+}$ & 9.983 & 9.999 &9.989& 10.001 &  9.990 & 9.982 & 9.990 & 9.976  & 9.998 & 9.987 \tabularnewline
			$2^{3}S_{1}$ & $1^{--}$ & 10.001 & 10.023 &10.017& 10.024  & 10.015 &  10.011 & 10.015  & 10.003  & 10.020 & 10.016\tabularnewline
			$3^{1}S_{0}$ & $0^{-+}$ & 10.342 &  & 10.336& 10.376 & 10.326 & 10.353 & 10.330  & 10.336 & 10.314 & 10.330 \tabularnewline
			$3^{3}S_{1}$ & $1^{--}$ & 10.354 & 10.355 &10.356& 10.392  &  10.343 & 10.373 & 10.349 & 10.354  & 10.334 & 10.351\tabularnewline
			$4^{1}S_{0}$ & $0^{-+}$ & 10.638 &  &10.597& 10.692 & 10.584 &  &  & 10.623  &  & 10.595 \tabularnewline
			$4^{3}S_{1}$ & $1^{--}$ & 10.650 & 10.579 &10.612& 10.705  & 10.597 & 10.654 & 10.607  & 10.635  &  & 10.611 \tabularnewline
			$5^{1}S_{0}$ & $0^{-+}$ & 10.901 & & 10.810& 10.981 &  10.800 &  &  & 10.869 &  & 10.817 \tabularnewline
			$5^{3}S_{1}$ & $1^{--}$ & 10.912 & 10.885 &10.822& 10.991  & 10.811 & 10.999 & 10.818  & 10.878  &  & 10.831 \tabularnewline
			$6^{1}S_{0}$ & $0^{-+}$ & 11.140 & & 10.991& 11.255 &  10.988 &  &  & 11.097 &  & 11.011 \tabularnewline
			$6^{3}S_{1}$ & $1^{--}$ & 11.151 & &11.001 & 11.308  &  10.997 & 11.265 & 10.995 & 11.102  &  & 11.023 \tabularnewline
			\addlinespace[1pt]
			\hline
			\addlinespace[3pt]
			$1^{3}P_{0}$ & $0^{++}$ & 9.874 & 9.859 &9.858& 9.857  & 9.864 &  9.851 & 9.855  & 9.847 & 9.865 & 9.865 \tabularnewline
			$1^{3}P_{1}$ & $1^{++}$ & 9.894 & 9.893 &9.889& 9.904  &  9.903 & 9.890 & 9.874 & 9.876  & 9.893 & 9.897 \tabularnewline
			$1^{1}P_{1}$ & $1^{+-}$ & 9.899 & 9.899 &9.894& 9.899 &  9.909 &  9.886 & 9.879 & 9.882  & 9.900 & 9.903 \tabularnewline
			$1^{3}P_{2}$ & $2^{++}$ & 9.907 & 9.912 &9.910& 9.919 & 9.921 & 9.899 & 9.886  & 9.897  & 9.913 & 9.918 \tabularnewline
			$2^{3}P_{0}$ & $0^{++}$ & 10.248 & 10.233 &10.235& 10.244  &  10.220 &  10.233 & 10.221 & 10.226  & 10.194 & 10.226 \tabularnewline
			$2^{3}P_{1}$ & $1^{++}$ & 10.265 & 10.255 &10.255& 10.276 & 10.249 & 10.257 & 10.236 & 10.246 & 10.212 & 10.251\tabularnewline
			$2^{1}P_{1}$ & $1^{+-}$ & 10.268 & 10.260 &10.259& 10.269  &  10.254 & 10.262 & 10.240 & 10.250  & 10.219 & 10.256 \tabularnewline
			$2^{3}P_{2}$ & $2^{++}$ & 10.274 & 10.269 &10.269& 10.287  &  10.264 & 10.274 & 10.246 & 10.261  & 10.227 & 10.269 \tabularnewline
			$3^{3}P_{0}$ & $0^{++}$ & 10.551 &  & 10.513&10.566 & 10.490 &  10.533 & 10.500  & 10.522 &  & 10.502 \tabularnewline
			$3^{3}P_{1}$ & $1^{++}$ & 10.567 & 10.512 &10.527& 10.590  &  10.515 &  10.556 & 10.513 & 10.538  &  & 10.524 \tabularnewline
			$3^{1}P_{1}$ & $1^{+-}$ & 10.570 &  & 10.530&10.561  & 10.519 & 10.560 & 10.516  & 10.541 &  & 10.529\tabularnewline
			$3^{3}P_{2}$ & $2^{++}$ & 10.576 & 10.524 & 10.539&10.600  & 10.528 &  10.568 & 10.521  & 10.550 &  & 10.540 \tabularnewline
			\addlinespace[1pt]
			\hline
			\addlinespace[3pt]
			$1^{3}D_{1}$ & $1^{--}$ & 10.145 &  & 10.153&10.151  & 10.146 & 10.136 & 10.117  & 10.138  & 10.150 & 10.145 \tabularnewline
			$1^{3}D_{2}$ & $2^{--}$ & 10.149 & 10.163 &10.162& 10.163  & 10.153 & 10.141 & 10.122  & 10.147  & 10.161 & 10.151\tabularnewline
			$1^{1}D_{2}$ & $2^{-+}$ & 10.149 &  &10.163& 10.161  & 10.153 &  & 10.123  & 10.148  & 10.163 & 10.152 \tabularnewline
			$1^{3}D_{3}$ & $3^{--}$ & 10.150 &  &10.170& 10.171  & 10.157 &  & 10.127  & 10.155 & 10.172 & 10.156\tabularnewline
			$2^{3}D_{1}$ & $1^{--}$ & 10.462 &  &10.442& 10.468  & 10.425 & 10.454 & 10.414  & 10.441  & 10.458 & 10.432 \tabularnewline
			$2^{3}D_{2}$ & $2^{--}$ & 10.465 &  &10.450& 10.479 & 10.432 &  & 10.418  & 10.449 & 10.401 & 10.438 \tabularnewline
			$2^{1}D_{2}$ & $2^{-+}$ & 10.465 &  & 10.450&10.479  &  10.432 &  & 10.419 & 10.450  & 10.447 & 10.439 \tabularnewline
			$2^{3}D_{3}$ & $3^{--}$ & 10.466 &  & 10.456&10.486 & 10.436 &  & 10.422  & 10.455  & 10.459 & 10.442 \tabularnewline
			$3^{3}D_{1}$ & $1^{--}$ & 10.736 & 10.752 &10.675& 10.757 &  & 10.725 & 10.653 & 10.698 &  & 10.670\tabularnewline
			$3^{3}D_{2}$ & $2^{--}$ & 10.740 &  &10.681& 10.766 &  &  & 10.657 & 10.705 &  & 10.676\tabularnewline
			$3^{1}D_{2}$ & $2^{-+}$ & 10.740 &  &10.681& 10.766 &  &  & 10.658 & 10.706 &  & 10.677\tabularnewline
			$3^{3}D_{3}$ & $3^{--}$ & 10.741 &  &10686& 10.773 &  &  & 10.660 & 10.711 &  & 10.680\tabularnewline
			$4^{3}D_{1}$ & $1^{--}$ & 10.985 & 11.000 &10.871 &11.028 & & &10.853 & 10.928& &10.877 \tabularnewline
			$4^{3}D_{2}$ & $2^{--}$ & 10.988 &  & 10.876&11.063 & & & &10.934 & &10.882 \tabularnewline
			$4^{1}D_{2}$ & $2^{-+}$ & 10.988 &  &10.876& 11.036 & & & &10.935 & &10.883 \tabularnewline
			$4^{3}D_{3}$ & $3^{--}$ & 10.990 &  &10.880& 11.041 & & & 10.860&10.939 & &10.886 \tabularnewline
			\hline
	\end{tabular}}
\end{table*}
